Effects of Naturalistic Variation in Goal-Oriented Dialog

Existing benchmarks used to evaluate the performance of end-to-end neural dialog systems lack a key component: natural variation present in human conversations. Most datasets are constructed through crowdsourcing, where the crowd workers follow a fixed template of instructions while enacting the role of a user/agent. This results in straight-forward, somewhat routine, and mostly trouble-free conversations, as crowd workers do not think to represent the full range of actions that occur naturally with real users. In this work, we investigate the impact of naturalistic variation on two goal-oriented datasets: bAbI dialog task and Stanford Multi-Domain Dataset (SMD). We also propose new and more effective testbeds for both datasets, by introducing naturalistic variation by the user. We observe that there is a significant drop in performance (more than 60% in Ent. F1 on SMD and 85% in per-dialog accuracy on bAbI task) of recent state-of-the-art end-to-end neural methods such as BossNet and GLMP on both datasets.

==> dataset-example.tex <==
\begin{table}[hbt!]
\centering
%
\footnotesize
%
\begin{tabular}{p{0.2cm}p{6.5cm}}
\toprule
\textbf{Dialogue$~$1$~$(D1)}                               &             \\
\midrule
\textbf{U}: & do you know about weather? \\
\textbf{A}: & yeah sure. You can ask me about weather for any location e.g. compton, manhattan, cleveland, inglewood etc. What would you like? \\
\textbf{U}: & what is the weather going to be today and tomorrow \\
\textbf{A}: & What city would you like to know the weather about? \\
\textbf{U}: & I want to know if it will drizzle in Durham \\
\textbf{A}: & It is not predicted to drizzle any today or tomorrow in Durham. \\
\textbf{U}: & Thank you \\
\textbf{A}: & anytime \\


\bottomrule
\end{tabular}
\caption{Sample dialog from SMD dataset between the User (\textbf{U}) and In-Car Assistant (\textbf{A}).}
\label{tab:dataset-samples}
\end{table}
